Environments of powerful radio galaxies through the cosmic ages

I define 3 samples of extragalactic radio sources of type FRII, containing 26 objects in total. The control sample consists of 6C and 7C sources with radio-luminosities of around 10E27 W\Hz at 151 MHz and z~1. The other samples contain 3CRR sources with either comparable redshifts but radio luminosities about a decade larger or with comparable radio-luminosities but redshifts around z~0.4. These samples are used to investigate the possible evolution of depolarisation and rotation measure properties with redshift and radio luminosity independently. I use the \citet{kat97} model with 3 flux measurements to estimate the density of the source environment, source age and jet power. Depolarisation and variations in the rotation measure were found to be insensitive to changes in the density of the source environment. This indicates that depolarisation and variations in the rotation measure are not density indicators but map how the disorder in the magnetic field changes with redshift. The model is then used on a larger set of FRII sources taken from the complete 3CRR, 6CE and 7C III samples. I find that the density of the source environment is a strong function of the source radio-luminosity but is insensitive to changes in redshift. The jet power is also a strong function of radio-luminosity but also a weak function of redshift. This indicates that the mass of the black-hole powering FRII sources is epoch dependent. In general, I find that the source environment is dominated by changes in the radio-luminosity but is relatively unaffected by changes in cosmic epoch.

==> abstract.tex <==
I define 3 samples of extragalactic radio sources of type FRII,
containing 26 objects in total. The control sample consists of 6C and
7C sources with radio--luminosities of around $10^{27}$\,W\,Hz$^{-1}$ at
151\,MHz and redshifts of $z\sim 1$. The other samples contain 3CRR
sources with either comparable redshifts but radio luminosities about a
decade larger or with comparable radio--luminosities but redshifts around
$z\sim 0.4$. These samples are used to investigate the possible
evolution of depolarisation and rotation measure properties with
redshift and radio luminosity independently.
% I used VLA data for all
%sources at $\sim$ 4800 MHz and two frequencies within the 1400 MHz
%band, either from my own observations or from the archive.  
All sources show evidence for an external Faraday screen.
% being responsible for the observed depolarisation. 
Depolarisation and variations in the rotation measure of a source
increase with redshift, only the depolarisation measure shows any
trend with radio-luminosity. There are no strong trends with spectral
index. \\ 
\indent I use the \citet{kat97} model with 3 flux measurements to estimate
the density of the source environment, source age and jet
power. Depolarisation and variations in the rotation measure were
found to be insensitive to changes in the density of the source
environment. This indicates that depolarisation and variations in the
rotation measure are not density indicators but map how the disorder
in the magnetic field changes with redshift.\\
\indent The model is then used on a larger set of FRII sources taken from 
the complete 3CRR, 6CE and 7C III samples. I find that the density of
the source environment is a strong function of the source
radio--luminosity but is insensitive to changes in redshift. The jet
power is also a strong function of radio-luminosity but also a weak
function of redshift. This indicates that the mass of the black--hole
powering FRII sources is epoch dependent. In general, I find that the
source environment is dominated by changes in the radio--luminosity
but is relatively unaffected by changes in cosmic epoch.

